Open-Vocabulary Semantic Part Segmentation of 3D Human

3D part segmentation is still an open problem in the field of 3D vision and AR/VR. Due to limited 3D labeled data, traditional supervised segmentation methods fall short in generalizing to unseen shapes and categories. Recently, the advancement in vision-language models' zero-shot abilities has brought a surge in open-world 3D segmentation methods. While these methods show promising results for 3D scenes or objects, they do not generalize well to 3D humans. In this paper, we present the first open-vocabulary segmentation method capable of handling 3D human. Our framework can segment the human category into desired fine-grained parts based on the textual prompt. We design a simple segmentation pipeline, leveraging SAM to generate multi-view proposals in 2D and proposing a novel HumanCLIP model to create unified embeddings for visual and textual inputs. Compared with existing pre-trained CLIP models, the HumanCLIP model yields more accurate embeddings for human-centric contents. We also design a simple-yet-effective MaskFusion module, which classifies and fuses multi-view features into 3D semantic masks without complex voting and grouping mechanisms. The design of decoupling mask proposals and text input also significantly boosts the efficiency of per-prompt inference. Experimental results on various 3D human datasets show that our method outperforms current state-of-the-art open-vocabulary 3D segmentation methods by a large margin. In addition, we show that our method can be directly applied to various 3D representations including meshes, point clouds, and 3D Gaussian Splatting.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% 3D part segmentation is important: enables machines with human-like ability: an parse objects into parts and generalize to unseen object and facilitates a wide range of applications, such as robotic manipulation, AR/VR, ...
The advancements in 3D technologies have led to an increased demand for automated analysis of 3D shapes. In particular, 3D part segmentation is an important task as it supports a wide spectrum of applications including robotic and AR/VR. 

% Human has more complex and varying geometry, richer semantic meanings, making it different from general object part segmentation
With the introduction of deep neural networks \cite{qi2017pointnet, qi2017pointnet++, thomas2019kpconv, xu2021paconv, zhao2021point, wang2019dynamic} and labeled 3D datasets \cite{wu20153d, chang2015shapenet, mo2019partnet}, 3D part segmentation has seen remarkable progress in recent years through supervised training. Nonetheless, due to limited data, enabling machines with human-like ability to parse objects into semantic parts and generalize to unseen object categories still remains difficult. This is especially the case with 3D humans, which contain more complex geometry with richer semantic attributes than general 3D objects.

% Current human part-specific segmentation run on 3D closed datasets, previous general 3D seg not working well on human data. these methods rely on a predefined set of semantic labels. Due to limited data, previous 3D-based methods are not generalizable to new categories and not suitable for human parts segmentation, which has highly variable combinations.
In contrast to generic shape data, there is also significantly fewer annotated data for 3D humans. Previous human parsing methods have been trained on clothed data \cite{bhatnagar2019multi, musoni2023gim3d, antic2024close}, but due to their inherent closed-set model structure, they can only parse humans into a predefined set of semantic labels. In addition, as existing datasets vary in terms of the labeled categories, content and quality, a model trained on one dataset may not generalize well to others. Although it is plausible to combine multiple datasets into a single taxonomy to enhance the generalization ability, the model will still remain inflexible to unseen classes and is hard to scale. 

% Recent developments in vision-language learning gave rise to many 2D image-based models with extreme zero-shot generalization capabilities. Many open-set segmentation methods are proposed to leverage the knowledge in 2D space. Most of them evaluated on object data and to the best of our knowledge, not working well for human. 
Recent developments in vision-language learning gave rise to many 2D image-based models \cite{radford2021learning, li2022grounded, jia2021scaling, zhai2023sigmoid} with exceptional zero-shot generalization capabilities. To extend to 3D, some works \cite{zhang2022pointclip, zhu2023pointclip, abdelreheem2023satr, liu2023partslip, zhou2023partslip++} have leveraged the knowledge of these models in 2D space and aggregate the multi-view information for the final segmentation result. While these methods have shown promising results on object data, they have not shown the same quality of results on 3D human data.

% we propose a way to transfer knowledge from 2D to 3D through SAM-based part segmentation on rendering and a novel lifting algorithm using finetuned to fuse inconsistent masks and build correlations with desired semantic labels
In this paper, we introduce the first open-vocabulary framework for 3D human parsing by transferring knowledge from 2D to 3D. As a mask-based segmentation method \cite{cheng2021per}, our method first applies SAM to rendered images and lifts to 3D to produce class-agnostic partial masks. In order to fuse the inconsistent masks and build correlations with the desired semantic labels, we leverage a novel HumanCLIP model to extract embeddings for each mask. Since this human-centric vision-language model can produce consistent embeddings for semantically similar masks, it helps with the seamless integration of inconsistent 3D masks. Our experimental results show our framework's flexibility to parse a 3D human with the desired labels and its generalizability to various 3D representations including meshes, point clouds, and 3D Gaussians \cite{kerbl20233d}.

% Efficient & flexible model design： one-time precomputed mask proposal supporting infinite segmentation
In summary, the main contributions of this work are:
\begin{itemize}
    \item The first open-vocabulary framework for 3D humans.
    \item A novel HumanCLIP model capable of extracting accurate CLIP embeddings for human parts.  
    \item Our framework demonstrates generalization ability to various 3D representations including meshes, point clouds, and 3D Gaussians.
\end{itemize}

==> sec/X_2_camera_sys.tex <==
\section{3D Mesh Generation from Multi-View Scans}

This section provides additional details about the process of obtaining in-the-wild mesh data for human subjects in the real world. 

\subsection{System Description}
Our capture system consists of four Intel RealSense D415 cameras positioned around the human subject. The cameras are placed in the north, south, east, and west directions relative to the subject, providing a full 360-degree view from the top of the head to the thighs and hip (see Figure \ref{fig:capturing-setup}). This arrangement allows for minimal occlusion, though the very top of the head is not visible. Each camera is connected to a central Windows computer, which coordinates the capture process using a Python program based on the RealSense SDK.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/capturing_setup.png}
    \caption{A picture showing the capturing setup, where the human subject is seated at the center and captures are taken by four surrounding Intel RealSense cameras.}
    \label{fig:capturing-setup}
\end{figure}

\subsection{RGB and Depth Image Capturing}

\subsubsection{Setup and Initialization of Cameras}

The cameras are configured to capture both RGB and depth images at a resolution of 640x480 pixels and a frame rate of 60 frames per second (FPS). The IR emitter and laser power are set to their maximum values.

\subsubsection{Synchronization and Warm-up}

Before capturing the actual data, the system performs a warm-up process for 2 minutes to stabilize the camera streams. During this period, a set number of frames are captured and discarded to allow the cameras to adjust to the environmental conditions.

\subsubsection{Image Capture}

For each capture session, the cameras are triggered simultaneously to ensure synchronized image acquisition. Each camera captures an RGB frame and a corresponding depth frame. The captured frames are then processed to align the RGB images to the depth images, ensuring that the color information corresponds accurately to the depth data.

\subsubsection{Depth Map Processing}

The captured frames undergo the following processing steps to improve the quality of the depth images and reduce noise.

\begin{itemize}
    \item Decimation Filter: to reduce the resolution of the depth image to remove noise and improve processing speed.
    \item Disparity Transform: The depth data is converted to disparity space for more effective filtering.
    \item Spatial Filter: to smooth the depth image by reducing spatial noise.
    \item Temporal Filter: to reduce temporal noise by averaging multiple frames.
    \item Disparity Transform (Inverse): The processed disparity data is converted back to depth space.
\end{itemize}


In addition to these filters, the RealSense SDK is configured to generate a normal vector for each point in the depth map, which will be used to generate a mesh. After processing, the RGB and depth images, along with the computed normal vectors, are saved to the disk.

\subsection{Camera Calibration}

For camera calibration, we utilize a ChArUco board with an 8x11 grid and a checkerboard size of 60 mm as shown in Figure \ref{fig:calibration-setup}. For each pair of adjacent cameras, we capture 20 images of the ChArUco board from different angles and positions. Given that the four cameras surround the human subject, every camera has two other cameras adjacent to it. Therefore, the total number of pairs of cameras is four.\\

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/calibration_setup.png}
    \caption{A picture showing two adjacent RealSense cameras facing a ChArUco board. The images of the ChArUco board taken from these two cameras will be used to find the relative rotation and translation between them.}
    \label{fig:calibration-setup}
\end{figure}

The captured images are processed to detect ChArUco markers, using the ChArUco detector in OpenCV. The stereo-calibration involves computing the rotation and translation matrices using the positions of the ChArUco markers in corresponding images between each pair of cameras, and this is performed using OpenCV. Bundle adjustment is performed to optimize the computed rotation and translation by minimizing the reprojection error.\\

The system chooses the viewpoint of one of the cameras as the world frame, and the point clouds obtained from each camera will be transformed to this world frame. Once the adjacent pairs are calibrated, the system computes the global calibration by finding the relative transformation between each camera and the world frame. A schematic diagram showing the stereo-calibration pipeline is shown in Figure \ref{fig:capturing-pipeline}.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/calibration_pipeline.png}
    \caption{The stereo-calibration pipeline to retrieve the transformation of each camera in the world frame.}
    \label{fig:capturing-pipeline}
\end{figure}

\subsection{Mesh Generation and Filtering}

After capturing RGB and depth frames from each camera and obtaining their relative transformations, the next step is to combine the point clouds from each camera to create a unified point cloud and subsequently generate a mesh. Prior to generating point clouds, the depth maps are processed to remove noise on the border of the subject, by the following steps:

\begin{itemize}
    \item Depth values outside a specified range (0.1 to 1.5 meters) are dropped to remove unwanted items that are not part of the human model.
    \item The depth map is converted to a grayscale image and filtered using a mode filter to smooth out small variations.
    \item A binary mask is created to identify the main object and remove small noise regions.
\end{itemize}

\subsubsection{Point Cloud Extraction}

For each camera, the depth map is converted into a point cloud. This involves mapping each pixel $(u, v)$ in the depth image to a 3D point $(X, Y, Z)$ in the camera coordinate system using the intrinsic parameters (focal length $f_x$, $f_y$ and image center $c_x$, $c_y$). 

$$X = \frac{(u - c_x)\cdot Z}{f_x}$$
$$Y = \frac{(u - c_y)\cdot Z}{f_y}$$
$$Z = \text{depth}(u,v)$$

The RGB values from the color images are associated with each 3D point to provide color information. Each point cloud is transformed into a global coordinate system using the rotation and translation matrices obtained from the calibration process.

$$\mathbf{p}_{\text{global}} = \mathbf{R} \mathbf{p}_{\text{local}} + \mathbf{t}$$

Here, $\mathbf{p}_{\text{local}}$ is a point in the camera's coordinate system, $\mathbf{R}$ is the rotation matrix, and $\mathbf{t}$ is the translation vector.

\subsubsection{Point Cloud Processing}

To remove noise from the combined point cloud, we apply a radius outlier removal filter. This filter eliminates points that have fewer than a specified number of neighbors within a given radius, effectively removing isolated points that are likely to be noise.

\subsubsection{Mesh Generation}

The filtered point cloud is used to generate a mesh using the Poisson surface reconstruction method. The generated mesh is smoothed using a simple Laplacian filter to reduce high-frequency noise. The colors of the mesh vertices are adjusted to match the colors from the original point cloud. A $k$-decision tree is used to find the nearest neighbors in the point cloud for each vertex in the mesh, and the color is interpolated accordingly. The resulting mesh can then be saved to a .ply file and visualized.
